Collage: Light-Weight Low-Precision Strategy for LLM Training

Large models training is plagued by the intense compute cost and limited hardware memory. A practical solution is low-precision representation but is troubled by loss in numerical accuracy and unstable training rendering the model less useful. We argue that low-precision floating points can perform well provided the error is properly compensated at the critical locations in the training process. We propose Collage which utilizes multi-component float representation in low-precision to accurately perform operations with numerical errors accounted. To understand the impact of imprecision to training, we propose a simple and novel metric which tracks the lost information during training as well as differentiates various precision strategies. Our method works with commonly used low-precision such as half-precision ($16$-bit floating points) and can be naturally extended to work with even lower precision such as $8$-bit. Experimental results show that pre-training using Collage removes the requirement of using $32$-bit floating-point copies of the model and attains similar/better training performance compared to $(16, 32)$-bit mixed-precision strategy, with up to $3.7\times$ speedup and $\sim 15\%$ to $23\%$ less memory usage in practice.

==> mcf_algos/Mul.tex <==
\begin{algorithm}[H]
\caption{\textbf{Mul} }
\label{alg:multmcn}
    \begin{algorithmic}
        \STATE {\bfseries Input:} $nc$-MCTensor $x, y$
        \STATE\bfseries{initialize:} $p\leftarrow \textbf{fl}(x_0\cdot y_0), \space  h_0\leftarrow p$
        \FOR{$i=1$ to $nc$}
        \STATE $e\leftarrow \textbf{Add-MCN}(x, -\textbf{DivN}(p, y))$
        \STATE $x\leftarrow e$
        \STATE $p\leftarrow \textbf{fl}(x_0 \cdot y_0)$
        \STATE $h_i\leftarrow p$
        \ENDFOR
        \STATE $h  \leftarrow (h_0, h_{1},\cdots, h_{nc})$
        \STATE {\bfseries Return:} \textbf{Simple-Renorm}$(h, nc)$
    \end{algorithmic}
\end{algorithm}

==> mcf_algos/Scaling.tex <==
\begin{algorithm}[H]
   \caption{\textbf{Scaling}, modified from \cite{shewchuk1997adaptive}}
   \label{alg:scaling}
    \begin{algorithmic}
    \STATE {\bfseries Input:}  $nc$-MCTensor $x$,\space  PyTorch Tensor $v$, \space $expand$
   \STATE \textbf{initialize} $e \leftarrow 0$
   \FOR{$i=0$ to $nc-1$}
   \STATE $(h_p, e_1) \leftarrow \textbf{Two-Prod}(x_{i}, v)$
   \STATE $(h_i, e_2) \leftarrow \textbf{Two-Sum}(h_{p}, e)$
   \STATE $e \leftarrow  \textbf{fl}(e_1+e_2) $
   \ENDFOR
    \STATE $h  \leftarrow (h_0, \cdots,h_{nc-1},e)$
\end{algorithmic}
\end{algorithm}
 

==> mcf_algos/Split.tex <==
\begin{algorithm}[H]
        \caption{\textbf{Split}}
        \label{alg:split}
        \begin{algorithmic}
          \STATE {\bfseries Input:} PyTorch Tensor $a$
          \IF{$a.dtype$ is HalfTensor (float16)} 
          \STATE $constant\leftarrow 6$
          \ELSIF{$a.dtype$ is FloatTensor (float32)}
          \STATE $constant\leftarrow 12$
          \ELSIF{$a.dtype$ is DoubleTensor (float64)}
          \STATE $constant\leftarrow 26$
          \ENDIF
          \STATE $t\leftarrow\textbf{fl}(2^{constant} + 1)\cdot a$
          \STATE $a_{hi}\leftarrow \textbf{fl}(t- \textbf{fl}(t-a))$
          \STATE $a_{lo}\leftarrow \textbf{fl}(a - a_{hi})$
           \STATE {\bfseries Return:} $(a_{hi}, a_{lo})$
        \end{algorithmic}
\end{algorithm}

==> mcf_algos/TwoProd.tex <==
\begin{algorithm}[H]
        \caption{\textbf{Two-Prod}}
        \label{alg:twoprod}
        \begin{algorithmic}
          \STATE {\bfseries Input:} PyTorch Tensors $a$, $b$
          \STATE $p\leftarrow \textbf{fl}(a \cdot b)$
          \STATE $(a_{hi}, a_{lo})\leftarrow\textbf{Split}(a)$
          \STATE $(b_{hi}, b_{lo})\leftarrow\textbf{Split}(b)$
          \STATE $err_1\leftarrow \textbf{fl}(p -  \textbf{fl}(a_{hi}\cdot b_{hi}))$
          \STATE $err_2\leftarrow \textbf{fl}(err_1- \textbf{fl}(a_{lo}\cdot b_{hi}))$
          \STATE $err_3\leftarrow \textbf{fl}(err_2- \textbf{fl}(a_{hi}\cdot b_{lo}))$
          \STATE $e\leftarrow \textbf{fl}(\textbf{fl}(a_{lo}\cdot b_{lo})-err_3)$
           \STATE {\bfseries Return:} $(p,e)$
        \end{algorithmic}
\end{algorithm}

==> mcf_algos/TwoProdFMA.tex <==
\begin{algorithm}[H]
        \caption{\textbf{Two-Prod-fma}}
        \label{alg:twoprodfma}
        \begin{algorithmic}
          \STATE {\bfseries Input:} PyTorch Tensors $a$, $b$ 
          \STATE {\bfseries Requires:} Machine supports FMA instructions set
          \STATE $p\leftarrow \textbf{fl}(a \cdot b)$
          \STATE $e\leftarrow$ torch.addcmul($-p, a, b$)
           \STATE {\bfseries Return:} $(p,e)$
        \end{algorithmic}
\end{algorithm}

==> mcf_algos/TwoSum.tex <==
\begin{algorithm}[H]
        \caption{\textbf{Two-Sum}}
        \label{alg:twosum}
        \begin{algorithmic}
          \STATE {\bfseries Input:} PyTorch Tensors $a,b$ 
           \STATE $x\leftarrow a+b$
           \STATE $b_{\text{virtual}}\leftarrow \textbf{fl}(x-a)$
           \STATE $a_{\text{virtual}}\leftarrow \textbf{fl}(x-b_{\text{virtual}})$
          \STATE $b_{\text{roundoff}}\leftarrow \textbf{fl}(b-b_{\text{virtual}})$
          \STATE $a_{\text{roundoff}}\leftarrow \textbf{fl}(a-a_{\text{virtual}})$
          \STATE $y\leftarrow \textbf{fl}(a_{\text{roundoff}}+b_{\text{roundoff}})$
            % \STATE $y\leftarrow ( (a - a_{\text{virtual}}) - \textbf{fl}(b - b_{\text{virtual}}))$
           \STATE {\bfseries Return:} $(x,y)$
        \end{algorithmic}
\end{algorithm}
